PANDA: Prompt Transfer Meets Knowledge Distillation for Efficient Model Adaptation

Prompt Transfer (PoT) is a recently-proposed approach to improve prompt-tuning, by initializing the target prompt with the existing prompt trained on similar source tasks. However, such a vanilla PoT approach usually achieves sub-optimal performance, as (i) the PoT is sensitive to the similarity of source-target pair and (ii) directly fine-tuning the prompt initialized with source prompt on target task might lead to forgetting of the useful general knowledge learned from source task. To tackle these issues, we propose a new metric to accurately predict the prompt transferability (regarding (i)), and a novel PoT approach (namely PANDA) that leverages the knowledge distillation technique to alleviate the knowledge forgetting effectively (regarding (ii)). Extensive and systematic experiments on 189 combinations of 21 source and 9 target datasets across 5 scales of PLMs demonstrate that: 1) our proposed metric works well to predict the prompt transferability; 2) our PANDA consistently outperforms the vanilla PoT approach by 2.3% average score (up to 24.1%) among all tasks and model sizes; 3) with our PANDA approach, prompt-tuning can achieve competitive and even better performance than model-tuning in various PLM scales scenarios. We have publicly released our code in https://github.com/WHU-ZQH/PANDA.

==> Tables_and_Figures/main-results.tex <==
\begin{table*}[]
\centering
\setlength{\tabcolsep}{10.5pt}
\scalebox{1}
{
\begin{tabular}{llccccccccl}
\toprule
\textbf{Method}        &
 \textbf{CB}   &
 \textbf{COPA} &
 \textbf{WSC}  &
 \textbf{RTE}  &
 \textbf{WIC}  &
 \textbf{CoLA} &
 \textbf{MRPC} &
 \textbf{STSB} &
%  \makebox[0.1\textwidth][l]{\footnotesize \textbf{CoNLL04}}
\textbf{CoNLL04} &
\textbf{AVG.}                     \\ 
% \midrule
%  \textbf{Metric}        &
%  \textbf{Acc.}   &
%  \textbf{Acc.} &
%  \textbf{Acc.}  &
%  \textbf{Acc.}  &
%  \textbf{Acc.}  &
%  \textbf{Mcc.} &
%  \textbf{Acc.} &
%  \textbf{Scor.} &
%  \textbf{F1.} &  
%  \; {--}\\
 \midrule \midrule
model-tuning   &
 94.6          &
 69.0          &
 68.3          &
 75.8          &
 74.9          &
 60.6          &
 88.0          &
 90.0          &
 85.6             &
 78.5                                  \\
\zqh{Lester et al.~\cite{lester2021power}}   &
\zqh{78.6}          &
\zqh{68.0}          &
\zqh{63.5}          &
\zqh{60.6}          &
\zqh{62.4}          &
\zqh{43.1}          &
\zqh{76.3}          &
\zqh{86.1}          &
\zqh{81.9}             &
\zqh{68.9}                                  \\
\zqh{P-Tuning-v2~\cite{liu2021p}}   &
 87.5          &
 76.0          &
 64.4          &
 76.2          &
 66.9          &
 63.8          &
 86.8          &
 90.5          &
 85.5             &
 77.5                                  \\ \midrule
\multicolumn{11}{c}{(a) Transfer with Vanilla Prompt Transfer approach~\cite{vu2021spot}. \zqh{P-Tuning-v2 is used for prompt-tuning in PoT.}}                                                                                                                                                          \\ \midrule
 MNLI      &
 \textbf{96.4} &
 71.0          &
 \textbf{67.3} &
 \textbf{80.9} &
 66.5          &
 58.9          &
 \textbf{88.2} &
 \textbf{91.0} &
 83.0             &
 \cellcolor[HTML]{FFFFFF}\textbf{78.1} \\
 QNLI      &
 \textbf{89.3} &
 76.0          &
 \textbf{65.4} &
 76.2          &
 \textbf{70.4} &
 63.7          &
 \textbf{88.5} &
 \textbf{90.7} &
 83.5             &
 \cellcolor[HTML]{FFFFFF}\textbf{78.2} \\ 
 Record    &
 78.6          &
 63.0          &
 \textbf{65.4} &
 53.8          &
 51.7          &
 0.0           &
 77.7          &
 85.0          &
 82.7             &
 62.0                                  \\
 SQuAD     &
 87.5          &
 74.0          &
 \textbf{66.3} &
 71.8          &
 51.7          &
 6.0           &
 \textbf{87.3} &
 89.3          &
 82.5             &
 68.5                                  \\ 
 CoNLL03   &
 73.2          &
 64.0          &
 63.5          &
 60.3          &
 51.9          &
 0.0           &
 71.3          &
 16.4          &
 84.8             &
 53.9                                  \\ 
 Ontonotes &
 78.6          &
 65.0          &
 \textbf{66.3} &
 56.7          &
 54.1          &
 59.3          &
 82.4          &
 84.5          &
 \textbf{86.1}    &
 70.3                                  \\ 
 CoNLL05   &
 87.5          &
 65.0          &
 64.4          &
 69.3          &
 \textbf{68.3} &
 61.3          &
 \textbf{88.7} &
 88.4          &
 83.8             &
 75.2                                  \\ 
 CoNLL12   &
 \textbf{89.3} &
 62.0          &
 \textbf{67.3} &
 63.2          &
 \textbf{67.4} &
 58.7          &
 90.4          &
 88.5          &
 83.6             &
 74.5                                  \\ 
 SST2      &
 \textbf{92.9} &
 74.0          &
 64.4          &
 71.8          &
 66.8          &
 60.1          &
 \textbf{87.0} &
 89.6          &
 84.3             &
 76.8                                  \\  
\hdashline
\multicolumn{11}{l}{\textit{Best transfer results of the vanilla prompt transfer}} \\
 ORACLE&96.4 &74.0 &67.3 &80.9 &70.4 &63.7 &88.7 &91.0 &86.1 &\cellcolor[HTML]{FFFFFF}\textbf{79.8} \\
 \hdashline
\multicolumn{11}{l}{\textit{Best of Top-3 transfer results predicted by ``E$_{avg}$'' metric in SPoT~\cite{vu2021spot}. }} \\
-w ``E$_{avg}$'' &96.4 &71.0 &67.3 &80.9 &66.8 &61.3 &88.5 &91.0 &86.1 &\cellcolor[HTML]{FFFFFF}\textbf{78.8} \\
 \midrule 
\multicolumn{11}{c}{(b) Transfer with Our \our approach. \zqh{P-Tuning-v2 is used for prompt-tuning in PoT.}}   \\ \midrule
 MNLI      &
 \textbf{92.9} &
 \textbf{77.0} &
 \textbf{67.3} &
 \textbf{78.0} &
 \textbf{68.8} &
 \textbf{66.3} &
 \textbf{88.5} &
 \textbf{90.6} &
 85.4             &
 \cellcolor[HTML]{FFFFFF}\textbf{79.4}$\boldsymbol{_{1.3}}$   \\
 QNLI      &
 \textbf{92.9} &
 \textbf{77.0} &
 \textbf{66.3} &
 \textbf{77.3} &
 \textbf{70.8} &
 63.9          &
 \textbf{87.5} &
 \textbf{90.8} &
 \textbf{86.6}    &
 \cellcolor[HTML]{FFFFFF}\textbf{79.2}$\boldsymbol{_{1.0}}$  \\
 Record    &
 87.5          &
 76.0          &
 \textbf{66.3} &
 \textbf{77.3} &
 \textbf{68.5} &
 62.4          &
 \textbf{87.5} &
 \textbf{90.7} &
 84.9             &
 \cellcolor[HTML]{FFFFFF}\textbf{77.9}$\boldsymbol{_{15.9}}$  \\
 SQuAD     &
 \textbf{89.3} &
 75.0          &
 \textbf{66.3} &
 75.5          &
 \textbf{69.3} &
 63.1          &
 \textbf{87.3} &
 88.9          &
 \textbf{85.7}    &
 \cellcolor[HTML]{FFFFFF}\textbf{77.8}$\boldsymbol{_{9.3}}$ \\
  CoNLL03   &
 \textbf{91.1} &
 72.0          &
 \textbf{68.3} &
 \textbf{76.9} &
 \textbf{67.4} &
 63.6          &
 86.5          &
 \textbf{90.6} &
 \textbf{85.6}    &
 \cellcolor[HTML]{FFFFFF}\textbf{78.0}$\boldsymbol{_{24.1}}$ \\
 Ontonotes &
 \textbf{89.3} &
 74.0          &
 \textbf{66.3} &
 76.2          &
 \textbf{69.1} &
 \textbf{64.2} &
 \textbf{88.0} &
 \textbf{90.8} &
 \textbf{85.7}    &
 \cellcolor[HTML]{FFFFFF}\textbf{78.2}$\boldsymbol{_{7.8}}$ \\
 CoNLL05   &
 87.5          &
 \textbf{79.0} &
 \textbf{65.4} &
 \textbf{77.6} &
 \textbf{69.6} &
 \textbf{63.7} &
 \textbf{87.5} &
 \textbf{90.8} &
 84.8             &
 \cellcolor[HTML]{FFFFFF}\textbf{78.4}$\boldsymbol{_{3.2}}$ \\
 CoNLL12   &
 87.5          &
 76.0          &
 \textbf{66.3} &
 74.4          &
 \textbf{68.5} &
 \textbf{63.7} &
 \textbf{87.5} &
 \textbf{90.8} &
 85.0             &
 \cellcolor[HTML]{FFFFFF}\textbf{77.7}$\boldsymbol{_{3.3}}$ \\
 SST2      &
 \textbf{92.9} &
 \textbf{77.0} &
 \textbf{68.3} &
 \textbf{76.5} &
 \textbf{70.1} &
 \textbf{64.8} &
 \textbf{88.5} &
 \textbf{90.7} &
 \textbf{86.3}    &
 \cellcolor[HTML]{FFFFFF}\textbf{79.5}$\boldsymbol{_{2.7}}$ \\
 \hdashline
 \multicolumn{11}{l}{\textit{Best transfer results of our \our approach}} \\
 ORACLE &92.9 &79.0 &68.3 &78.0 &70.8 &66.3 &88.5 &90.8 &86.6 &\cellcolor[HTML]{FFFFFF}\textbf{80.1}$\boldsymbol{_{0.3}}$ \\
  \hdashline
\multicolumn{11}{l}{\textit{Best of Top-3 transfer results predicted by our metric. }} \\
-w Ours &92.9 &77.0 &68.3 &78.0 &70.8 &66.3 &88.5 &90.8 &85.7 &\cellcolor[HTML]{FFFFFF}\textbf{79.8}$\boldsymbol{_{1.0}}$ \\
 \bottomrule
\end{tabular}
}
\caption{Results (\%) of part of cross-tasks PoT based on BERT-large model (full results can be seen in Table~\ref{tab:results_large}).
In the groups of (a) and (b), each cell denotes the target task performance when transferring the prompt from source task (row) to the associated target task (column).
``AVG.'' denotes the average performance of all target tasks. Notably, positive prompt transfers are in \textbf{bold} and numbers in the subscript indicate relative improvements of our \our against vanilla PoT.}
\label{tab:main}
\end{table*}

